The Restricted Isometry Property of Block Diagonal Matrices for Group-Sparse Signal Recovery

Group-sparsity is a common low-complexity signal model with widespread application across various domains of science and engineering. The recovery of such signal ensembles from compressive measurements has been extensively studied in the literature under the assumption that measurement operators are modeled as densely populated random matrices. In this paper, we turn our attention to an acquisition model intended to ease the energy consumption of sensing devices by splitting the measurements up into distinct signal blocks. More precisely, we present uniform guarantees for group-sparse signal recovery in the scenario where a number of sensors obtain independent partial signal observations modeled by block diagonal measurement matrices. We establish a group-sparse variant of the classical restricted isometry property for block diagonal sensing matrices acting on group-sparse vectors, and provide conditions under which subgaussian block diagonal random matrices satisfy this group-RIP with high probability. Two different scenarios are considered in particular. In the first scenario, we assume that each sensor is equipped with an independently drawn measurement matrix. We later lift this requirement by considering measurement matrices with constant block diagonal entries. In other words, every sensor is equipped with a copy of the same prototype matrix. The problem of establishing the group-RIP is cast into a form in which one needs to establish the concentration behavior of the suprema of chaos processes which involves estimating Talagrand's $\gamma_2$ functional. As a side effect of the proof, we present an extension to Maurey's empirical method to provide new bounds on the covering number of sets consisting of finite convex combinations of possibly infinite sets.

==> blacronyms.tex <==
\newacronym{ADC}{ADC}{analog-to-digital converter}
\newacronym{ADMM}{ADMM}{alternating direction method of multipliers}
\newacronym{AMP}{AMP}{approximate message passing}
\newacronym{AOP}{AOP}{adaptive outlier pursuit}
\newacronym{BFCS}{BFCS}{binary fused compressive sensing}
\newacronym{BIHT}{BIHT}{binary iterative hard thresholding}
\newacronym{BOS}{BOS}{bounded orthonormal system}
\newacronym{BPDN}{BPDN}{basis pursuit denoising}
\newacronym{BP}{BP}{basis pursuit}
\newacronym{BRIC}{block-RIC}{block restricted isometry constant}
\newacronym{BRIP}{block-RIP}{block \acl{RIP}}
\newacronym{BSGF}{BSGF}{binary sparse group fusion}
\newacronym{BeSE}{B$\epsilon$SE}{binary epsilon stable embedding}
\newacronym{CS-BIHT}{CS-BIHT}{conjugate symmetric binary iterative hard thresholding}
\newacronym{CS}{CS}{compressed sensing}
\newacronym{CoSaMP}{CoSaMP}{compressive sampling matching pursuit}
\newacronym{DCS}{DCS}{distributed \acl{CS}}
\newacronym{DCT}{DCT}{discrete cosine transform}
\newacronym{DFT}{DFT}{discrete Fourier transform}
\newacronym{DOA}{DOA}{direction of arrival}
\newacronym{DVB-T}{DVB-T}{digital video broadcasting - terrestrial}
\newacronym{EM}{EM}{expectation maximization}
\newacronym{FDMA}{FDMA}{frequency-division multiple access}
\newacronym{FFT}{FFT}{fast Fourier transform}
\newacronym{FISTA}{FISTA}{fast iterative soft thresholding algorithm}
\newacronym{GNSP}{group-NSP}{group null space property}
\newacronym{GRIC}{group-RIC}{group restricted isometry constant}
\newacronym{GRIP}{group-RIP}{group \acl{RIP}}
\newacronym{HRA}{HRA}{high-resolution assumption}
\newacronym{HTP}{HTP}{hard thresholding pursuit}
\newacronym{IHT}{IHT}{iterative hard thresholding}
\newacronym{IRLS}{IRLS}{iteratively reweighted least-squares}
\newacronym{ISTA}{ISTA}{iterative soft thresholding algorithm}
\newacronym{IST}{IST}{iterative soft thresholding}
\newacronym{IoT}{IoT}{internet of things}
\newacronym{JSM2}{JSM-2}{joint sparsity model 2}
\newacronym{LASSO}{LASSO}{least-absolute shrinkage selection operator}
\newacronym{LP}{LP}{linear program}
\newacronym{MC}{MC}{Monte Carlo}
\newacronym{MGF}{MGF}{moment generating function}
\newacronym{MIMO}{MIMO}{multiple-input multiple-output}
\newacronym{MMV}{MMV}{multiple measurement vector}
\newacronym{MRIC}{model-RIC}{model \acl{RIC}}
\newacronym{MRIP}{model-RIP}{model \acl{RIP}}
\newacronym{MSE}{MSE}{mean square error}
\newacronym{MSP}{MSP}{matched sign pursuit}
\newacronym{NMSE}{NMSE}{normalized mean square error}
\newacronym{NSP}{NSP}{null space property}
\newacronym{OMP}{OMP}{orthogonal matching pursuit}
\newacronym{PBIBHT}{PBIBHT}{proximal binary iterative block hard thresholding}
\newacronym{QCBP}{QCBP}{quadratically-constrained basis pursuit}
\newacronym{QCS}{QCS}{quantized compressed sensing}
\newacronym{QIHT}{QIHT}{quantized iterative hard thresholding}
\newacronym{RFPI}{RFPI}{renormalized fixed-point iteration}
\newacronym{RIC}{RIC}{restricted isometry constant}
\newacronym{RIP}{RIP}{restricted isometry property}
\newacronym{RSS}{RSS}{restricted-step shrinkage}
\newacronym{RoBFCS}{RoBFCS}{robust binary fused compressive sensing}
\newacronym{SGFDN}{SGFDN}{sparse group fused denoising}
\newacronym{SGFLASSO}{SGF-LASSO}{sparse group fused LASSO}
\newacronym{SNR}{SNR}{signal-to-noise ratio}
\newacronym{SOCP}{SOCP}{second-order cone program}
\newacronym{SOS}{SOS}{sum-of-squares}
\newacronym{SPE}{SPE}{sign product embedding}
\newacronym{TV}{TV}{total variation}
\newacronym{UoS}{UoS}{union-of-subspaces}
\newacronym{fMRI}{fMRI}{functional magnetic resonance imaging}

